Geometric Losses for Distributional Learning

Building upon recent advances in entropy-regularized optimal transport, and upon Fenchel duality between measures and continuous functions , we propose a generalization of the logistic loss that incorporates a metric or cost between classes. Unlike previous attempts to use optimal transport distances for learning, our loss results in unconstrained convex objective functions, supports infinite (or very large) class spaces, and naturally defines a geometric generalization of the softmax operator. The geometric properties of this loss make it suitable for predicting sparse and singular distributions, for instance supported on curves or hyper-surfaces. We study the theoretical properties of our loss and show-case its effectiveness on two applications: ordinal regression and drawing generation.

==> old.tex <==
%!TEX root = article.tex
% \section{Convex losses for continuous prediction}\label{sec:background}

% To motivate our construction, it is useful to view the two functions of \autoref{def:layers} as counterpart of the well-known softmax operator and logsumexp in the discrete case, with no distance consideration in the output space. In our case, our model should predict a continuous probability measure in $\cM_1^+(\cY)$, instead of a histogram on the $d$-dimensional simplex $\Simplex^d$. Therefore, we start by recalling a generic way of building convex losses and predictors for discrete probability distribution.

% \subsection{Predicting discrete probabilities}



% \subsection{Cost-sensitive losses}

% \subsection{Continuous distribution prediction}

% Put here "A detour through Banach spaces"

% Wasserstein etc.

% \subsection{Fenchel-Young losses for discrete prediction}

% \paragraph{Going metric and infinite.}Our construction extends the existing framework to answer two natural questions. The existing analysis considers an output space $\cY$ without
% notion of distance between output classes. Can we define negative entropies that take
% into account a distance between classes $C: \cY \times \cY \to \RR$? More generally, can we work with infinite
% metrized output space $\cY$? To provide an answer,
% we now drop the discrete class assumption and consider a general compact metric space $\cY$ of output, equiped with a distance~$C$. Relying on topological duality, we construct the loss and link function from \autoref{def:layers} from negative entropies
% defined on the space $\cM_1^+(\cY)$, recently introduced by 
% \cite{ramdas_wasserstein_2015,feydy_interpolating_2018}. The general space of probability
% measure $\cM_1^+(\cY)$ is more complex than $\Simplex^d$, making the extension of the construction challenging. In particular, we would like to learn models that converge toward Bayes risk minimizer in the weak sense:

% \begin{equation}
%     g_{\theta_n}(x) \rightharpoonup g_{\theta^\star}(x)\quad\text{iff }
%     {\forall\,f \in \contspace}, \langle g_{\theta_n}(x), f \rangle
%     \to \langle g_{\theta^\star}(x), f \rangle
% \end{equation}

% This excludes the Kullback Liebler divergence, that is not defined
% on general spaces of probability measure, and metrizes the strong convergence on the subspace of $\probspace \times \probspace$ on which it is defined.


% The Fenchel-Young loss framework, predictors of probability distribution are defined with a component $\nabla \Omega^\star$, that is a mirror map in between the dual space of probability distribution $\Simplex^d$ and the primal space of score $\RR^d$.
